Diagnosis via Proofs of Unsatisfiability for First-Order Logic with Relational Objects

Satisfiability-based automated reasoning is an approach that is being successfully used in software engineering to validate complex software, including for safety-critical systems. Such reasoning underlies many validation activities, from requirements analysis to design consistency to test coverage. While generally effective, the back-end constraint solvers are often complex and inevitably error-prone, which threatens the soundness of their application. Thus, such solvers need to be validated, which includes checking correctness and explaining (un)satisfiability results returned by them. In this work, we consider satisfiability analysis based on First-Order Logic with relational objects (FOL*) which has been shown to be effective for reasoning about time- and data-sensitive early system designs. We tackle the challenge of validating the correctness of FOL* unsatisfiability results and deriving diagnoses to explain the causes of the unsatisfiability. Inspired by the concept of proofs of UNSAT from SAT/SMT solvers, we define a proof format and proof rules to track the solvers' reasoning steps as sequences of derivations towards UNSAT. We also propose an algorithm to verify the correctness of FOL* proofs while filtering unnecessary derivations and develop a proof-based diagnosis to explain the cause of unsatisfiability. We implemented the proposed proof support on top of the state-of-the-art FOL* satisfiability checker to generate proofs of UNSAT and validated our approach by applying the proof-based diagnoses to explain the causes of well-formedness issues of normative requirements of software systems.

==> archive/BIGTABLE.tex <==
\begin{table}[t]
    \centering
    \caption{Effectiveness of \approach for triming UNSAT proofs. 
    For each generated UNSAT proof of well-formedness property, the initial (init.) proof file size in Kilobyte (size) with the number of proof derivation steps (n-steps), as well as the proof file size and the number of steps remaining after checking the proof (check.).
    %Volume differences between $\opt$ and $\noopt$ are bolded. 
    }
    \label{tab:effectiveness}
    % time without time with initial step, steps after checking, steps once minimized
    \scalebox{0.8}{
    \begin{tabular}{r ccccc c ccccc c ccccc c ccccc}
        \toprule
         & \multicolumn{23}{c}{well-formedness property}\\\cmidrule{2-24}
        & \multicolumn{5}{c}{conflict} & ~ & \multicolumn{5}{c}{s-conflict} && \multicolumn{5}{c}{redundancy} && \multicolumn{5}{c}{restrictiveness}\\\cmidrule{2-6}\cmidrule{8-12}\cmidrule{14-18}\cmidrule{20-24}
         \multirow{2}{*}{case studies} & \multirow{1}{*}{over.} & \multicolumn{2}{c}{initial} & \multicolumn{2}{c}{check.} & & \multirow{1}{*}{over.} & \multicolumn{2}{c}{initial} & \multicolumn{2}{c}{check.} && \multirow{1}{*}{over.} & \multicolumn{2}{c}{initial} & \multicolumn{2}{c}{check.} && \multirow{1}{*}{over.} & \multicolumn{2}{c}{initial} & \multicolumn{2}{c}{check.}\\\cmidrule{3-6}\cmidrule{9-12}\cmidrule{15-18}\cmidrule{21-24}
         &  & size & n-steps & size & n-steps & & & size & n-steps &  size & n-steps & & & size & n-steps &  size & n-steps & & &size & n-steps &  size & n-steps \\
         \toprule 
            % ALMI ------------
            \cellcolor{gray!30}  ALMI & \multicolumn{5}{c}{satisfiable} &~& 0.13 & 256 & 664 & 104 & 137 &~& \multicolumn{5}{c}{satisfiable}  &~& \multicolumn{5}{c}{satisfiable} \\\midrule
            % ASPEN ------------
              ASPEN &\multicolumn{5}{c}{satisfiable} &~& 0.26 & 392 & 1607 & 76 & 118 &~& 0.08 & 151 & 751 & 27 & 101 &~& \multicolumn{5}{c}{satisfiable}\\
             %----
              &\multicolumn{5}{c}{~} &~& 0.21 & 230 & 745 & 76 & 111 &~&  &  &  &  &  &~& \multicolumn{5}{c}{~}\\
             %----
              &\multicolumn{5}{c}{~} &~& -0.05 & 268 & 832 & 76 & 111 &~&  &  &  &  &  &~& \multicolumn{5}{c}{~}\\\midrule
            % Autocar ------------
             AutoCar & \multicolumn{5}{c}{satisfiable} &~&  \multicolumn{5}{c}{satisfiable} &~& 0.21 & 143 & 576 & 29 & 97 &~& \multicolumn{5}{c}{satisfiable}\\
             %---
             & \multicolumn{5}{c}{~} &~&  \multicolumn{5}{c}{~} &~& 0.21 & 159 & 673 & 29 & 97 &~& \multicolumn{5}{c}{~}\\\midrule
             %BSN & \multicolumn{5}{c}{satisfiable} &~& \multicolumn{5}{c}{satisfiable} &~& o & s & ss & s & ss &~& o & s & ss & s & ss\\
            % Casper ------------
             Casper & \multicolumn{5}{c}{satisfiable} &~& \multicolumn{5}{c}{satisfiable} &~& 0.17 & 85 & 320 & 23 & 94 &~& \multicolumn{5}{c}{satisfiable}\\\midrule 
            % CSI ------------
             CSI-Cobot & \multicolumn{5}{c}{satisfiable} &~& \multicolumn{5}{c}{satisfiable} &~& 0.12 & 34 & 131 & 88 & 51 &~& \multicolumn{5}{c}{satisfiable}\\
             %-- 
             & \multicolumn{5}{c}{~} &~& \multicolumn{5}{c}{~} &~& 0.12 & 35 & 131 & 9 & 51 &~& \multicolumn{5}{c}{~}\\
             & \multicolumn{5}{c}{~} &~& \multicolumn{5}{c}{~} &~& 0.13 & 52 & 228 & 97 & 53 &~& \multicolumn{5}{c}{~}\\\midrule  
            % DAISY ------------
             DAISY &  \multicolumn{5}{c}{satisfiable}  &~& 0.33 & 648 & 1854 & 118 & 122 &~& 0.15 & 48 & 136 & 7 & 30 &~& \multicolumn{5}{c}{satisfiable} \\
             &  \multicolumn{5}{c}{~}  &~& 0.29 & 520 & 1470 & 117 & 122 &~&  &  &  &  &  &~& \multicolumn{5}{c}{~} \\\midrule         
             % DPA ------------
             %DPA &  \multicolumn{5}{c}{satisfiable} &~& o & s & ss & s & ss &~& o & s & ss & s & ss &~& o & s & ss & s & ss\\ 
            % SafeSCAD ------------
             SafeSCAD &  \multicolumn{5}{c}{satisfiable}  &~& 0.25 & 234 & 648 & 74 & 116 &~& 0.02 & 39 & 155 & 9 & 51 &~& 0.04 & 43 & 162 & 10 & 53\\
             %--
             &  \multicolumn{5}{c}{~}  &~& 0.22 &  240 & 779 & 68 & 67 &~& 0.02 & 40 & 159 & 10 & 53 &~& 0.03 & 42 & 169 & 10 & 60\\
             %--
             &  \multicolumn{5}{c}{~}  &~& 0.23 &  226 & 721 & 67 & 81 &~&  &  &  &  &  &~&  &  & & &\\
             %--
             &  \multicolumn{5}{c}{~}  &~& 2.25 &  244 & 843 & 88 & 162 &~&  &  &  &  &  &~&  &  & & &\\
             %--
             &  \multicolumn{5}{c}{~}  &~& 0.34 &  358 & 1175 & 100 & 204 &~&  &  &  &  &  &~&  &  & & &\\
             %--
             &  \multicolumn{5}{c}{~}  &~& 0.26 &  196 & 544 & 83 & 156 &~&  &  &  &  &  &~&  &  & & &\\
             %--
             &  \multicolumn{5}{c}{~}  &~& 0.29 &  236 & 793 & 88 & 162 &~&  &  &  &  &  &~&  &  & & &\\
             %--
             &  \multicolumn{5}{c}{~}  &~& 0.27 &  197 & 544 & 89 & 162 &~&  &  &  &  &  &~&  &  & & &\\
             %--
             &  \multicolumn{5}{c}{~}  &~& 0.32 &  248 & 674 & 101 & 207 &~&  &  &  &  &  &~&  &  & & &\\
             %--
             &  \multicolumn{5}{c}{~}  &~& 0.56 &  245 & 849 & 83 & 156 &~&  &  &  &  &  &~&  &  & & & \\
             %--
             &  \multicolumn{5}{c}{~}  &~& 0.33 &  263 & 769 & 101 & 207 &~&  &  &  &  &  &~&  &  & & &\\\midrule
             % Tabiat --------------
             Tabiat & -0.07 & 230 & 963 & 18 & 93 &~& 0.13 & 203 & 555 & 79 & 55 &~& 0.09 & 216 & 895 & 19 & 93 &~& 0.09 & 141 & 455 & 21 & 85\\
             %--
             & 0.05 & 133 & 398 & 18 & 73 &~& 0.13 & 232 & 586 & 71 & 34 &~& 0.09 & 50 & 165 & 9 & 44 &~& 0.1 & 236 & 1022 & 18 & 93\\
             %--
             & -0.04 & 256 & 1091 & 22 & 114 &~& 0.13 & 229 & 632 & 68 & 42 &~& 0.13 & 259 & 1089 & 14 & 73 &~& 0.11 & 237 & 1022 & 18 & 93\\
             %--
             & 0.03 & 233 & 963 & 18 & 93 &~& 0.14 & 199 & 542 & 90 & 105 &~& 0.12 & 231 & 945 & 19 & 93 &~&  &  &  &  & \\
             %--
             & 0.01 & 245 & 1028 & 18 & 93 &~& 0.13 & 200 & 542 & 91 & 105 &~& 0.09 & 233 & 947 & 19 & 93 &~&  &  &  &  &\\
             %--
             & -0.16 & 234 & 963 & 18 & 93 &~& 0.14 & 199 & 542 & 84 & 98 &~&  &  &  &  &  &~&  &  &  &  &\\
             %--
             &  & & &  & &~& 0.14 & 244 & 657 & 85 & 93 &~&  &  &  &  &  &~&  &  &  &  &\\
             %--
             &  & & &  & &~& 0.13 & 257 & 699 & 69 & 34 &~&  &  &  &  &  &~&  &  &  &  &\\
             %--
             &  & & &  & &~& -0.19 & 369 & 990 & 98 & 127 &~&  &  &  &  &  &~&  &  &  &  &\\
        \bottomrule
    \end{tabular}
    }
    %\vspace{-0.2in}
\end{table}

==> archive/approach.tex <==
\boldparagraph{\nf{Support for optimizations in algorithm \searcha}}
\nf{Below}, we describe \nf{how the optimizations are integrated in} \legos{} algorithm \searcha{}  shown in \hl{Alg}.~\ref{alg:main}.  Blue parts are specific to \legos{}, and black are taken from the \ibs{} algorithm \search. The optimized algorithm \searcha{} takes \nf{two} additional flags {\bf MC:  why three flags for two optimizations?} \blue{[corrected]}, $bcr$, and $t_{res}$ indicating whether optimizations ``boundary case reduction'' (BCR), and ``restart''($t_{res}$ defining the initial restart threshold, default is $\infty$) are enabled. BCR takes effect while grounding the \tfol{} formula $\phi$ (L:~\ref{ln:computeOverground}). \searcha{} has two search modes, relaxed and optimal (normal). It starts in a relaxed mode (L:~\ref{ln:relaxedinit}) that allows relaxed domain expansion optimizations~\ref{subsub:relaxed} (L:~\ref{ln:expandingdomain}). 
When \bunsat{} is detected during the relaxed mode, \searcha{} switches mode to the optimal search one
%instead of returning
%\bunsat, \searcha{} switches off the relaxed mode and continues in the
%optimal search mode 
(L:~\ref{ln:returnboundedUNSAT}). 
Before each
iteration (L:~\ref{ln:restart}), if the number of iterations since refining the last requirement is greater than a threshold value, ``restart'' takes effect and clears all requirements.  The value of $t_{res}$ are multiplied by $1.25$ every time ``restart''  takes place. \searcha{} returns \unsat{} under the same conditions as \search. However, \bunsat{} can only be returned in the optimal search mode. If optimality is required, then any solution produced during the relaxed mode needs to be minimized in the optimal search mode.
%
\nf{See Sec~\ref{ap:exampleAlg} for an illustration of $\mainAlg$.}
 



\begin{comment}
\subsubsection{Example. }
Consider the banking system that supports operations: \indent 1. A user $u$ can deposit $x$ amount of funds by deposit $\textit{DP}(u, x)$
\indent 2. A user $u$ can transfer $x$ amount of fund to a different user $v$ by transfer $\textit{TR}(u, v, x)$\\
A user's balance at time $t$ is defined as the sum of money deposited plus the sum of money transferred-in minus sum of money transferred-out: $\textit{Balance}(u, t) = \textit{Sum}(\textit{DP}, \lambda dp:\: dp.user = u \wedge dp.\textit{time} \le t, \lambda dp:\: dp.x) + \textit{Sum}(\textit{TR}, \lambda tr:\:tr.receiver = u \wedge tr.\textit{time} \le t, \lambda tr:\:tr.x) + \textit{Sum}(\textit{TR}, \lambda tr:\:tr.\textit{sender} = u \wedge tr.\textit{time} \le t, \lambda tr:\:tr.x)$

\noindent
The bank establishes the following requirements: (R1) A user can deposit at most $500$ every day.  (R2) A user can transfer $x$ amount of fund only if the user's balance is no less than $x$ before the transfer. (R3) A user can receive up to at most two transfers per day, (R4) but can only send a transfer once per day.

 Suppose that the banking system wants to check a security property to ensure that no user should accumulate more than 200,000 funds and transfer them out within the first 5 days. This could be formalized in \tfol{} as $\forall tr:TR. \neg (tr.x \ge 20000 \wedge Balance(tr.u, tr.time - 5) = 0)$. To check this property, its negation, $\exists tr:TR. (tr.x \ge 20000 \wedge tr.time \le 5)$, is asserted, and it in turn instantiate a relational objects $tr_1$ via grounding (Alg.~\ref{alg:ground}). For each iteration, we denote $\phi_g$ and $\phi_g^\bot$ as the over- and under-approximation queries computed on L:~\ref{ln:computeOverground} and L:~\ref{ln:computeUnderground} of Alg.~\ref{alg:main}, respectively. We also denote the over- and under-approximated sum values with $\textit{sum}^\uparrow$ and $\textit{sum}^\downarrow$, respectively. \\
%
\underline{Iteration 1.} $\domainUnder =  \{tr_1\}$. By R2, $tr_1$ requires a sufficient amount of balance of the sender before the transfer:  {\bf MC:  are we going to use Balance or balance to name this predicate?} $\textit{balance}(tr_1.\textit{sender}, tr_1.\textit{time}-1) \ge tr.x$ and $\textit{balance}(tr_1.\textit{sender}, tr_1.\textit{time}-1)$ can be expanded into three summations: $\textit{sum}_1 + \textit{sum}_2 - \textit{sum}_3$ where $\textit{sum}_1$, $\textit{sum}_2$ and $\textit{sum}_3$ are for the summation of the deposited, transferred-in, and transferred-out fund, respectively. Note that  $\textit{sum}_1^\downarrow$, $\textit{sum}_2^\downarrow$, and $\textit{sum}_3^\downarrow$ are 0 in $\domainUnder$. Therefore, $\phi_g^\bot$ is unsatisfiable as $\textit{balance}(\textit{tr.user}, tr.\textit{time}-1) = 0 < 10000$. However, $\phi_g$ is satisfiable, since a solution can be obtained by over-approximating the sum of  deposit as $\textit{sum}_1^{\uparrow} = 20000$. However,  $\textit{sum}_1\uparrow$, by $req_{\textit{sum}}$, has to introduce a new relational object "Deposit" $dp_1$ with constraints $dp_1 = tr_1.\textit{sender}$, $dp_1.x > 0$, $dp_1.\textit{time} < tr_1.\textit{time}$. A new summation $\textit{sum}_4$ is also introduced such that $\textit{sum}_4 = = \textit{sum}_1- dp_1.x $.  \\
\underline{Iteration 2} $\domainUnder =  \{tr_1, \textit{sum}_1, dp_1, \textit{sum}_4\}$. According to requirement R1, $dp_1.x \le 500$.  Therefore, $\textit{balance}(\textit{tr}_1.\textit{sender}, \textit{tr}_1.\textit{time}-1) \le 500$ in $\domainUnder$, and thus the $\phi_g^\bot$ is unsatisfiable. However, $\phi_g$ is satisfiable, since a  solution can be obtained with $\textit{sum}_4^{\uparrow} = 19500$. Note that $\textit{sum}_4^\uparrow$ has to introduce (by $req_{\textit{sum}}$) a new relational object $dp_2$ and a new sum $\textit{sum}_5 = \textit{sum}_4 - dp_2.x$ similar to iteration 1. As the next iteration progresses, more and more deposits and sums are introduced into the chain of relational objects to increase $\textit{balance}(tr_1.\textit{sender}, tr_1.\textit{time}-1)$. We now move on to Iteration 5.\\
%
\underline{Iteration 5} $D_{AU} =  \{tr_1, \textit{sum}_1, dp_1 ... dp_4, \textit{sum}_3... \textit{sum}_5 \}$. Note that $\textit{sum}_5^{\downarrow} \le 4 * 500 = 2000$, and $\phi_g^\bot$ is unsatisfiable.  On the other hand, $\textit{sum}_6^{\uparrow} \le 0$ due to R1 as $tr.send$ has already deposite 500 everyday via $dp_1 ... dp_4$. This implies that 20,000 funds cannot be accumulated by only depositing. However, $\phi_g$ is satisfiable, since a satisfying solution can be obtained by over-approximating the transferred-in sum $\textit{sum}_2^{\uparrow} = 18000$ to cover the discrepancy as $\textit{sum}_2^{\uparrow} + \textit{sum}_1^{\downarrow} = 20000$. By $req_{\textit{sum}}$, $\textit{sum}_2^{\uparrow}$ introduces a new relational object $tr_2$ where $tr_2.\textit{receiver} = tr_1.\textit{sender}$ and $tr_2.\textit{time} < tr_1.\textit{time}$.  The remaining sum is covered by a new sum $\textit{sum}_7 = \textit{sum}_2 - tr_2.x$. At the next iteration, (R2) would trigger another chain of events that introduces more transfer, deposit, and summation to increase the balance of $tr_2.\textit{sender}$. Now we proceed to the final iteration. \\
\underline{The final iterations}  $D_{AU} =  \{tr_1, tr_2 ... tr_19,  \textit{sum}_1, \textit{sum}_2, dp_1 ... dp_20, \textit{sum}_3... \}$, the under-approximated query has a solution.The solution involves 27 users. On the first day, all users deposit 500. On the second day, users are divided into 9 groups of 3s, two users transfer all of their balance to the third user while the third user keeps depositing. We keep only the third user for each group. On day two, the 9 remaining users can each accumulate 2000 fund. On day three, among the 9 users, we form 3 groups of threes, and perform the same operation as day 2, and the remaining 3 users can accumulate 6500 fund. On day 4, $tr_2.\textit{sender}$ keeps depositing, while the remaining two users transfer all its balance. The balance of $tr_2.\textit{sender}$ on day 4 is 20000, which allows him transfer all of them out on day 5. Therefore, the security properties might be violated under the current set of requirements. On the other hand, if we tighten the requirements by restricting the amount of deposit to be less than 500 every time, then our tools shows the security property cannot be violated.
\end{comment}
\begin{comment}

\subsection{Implementation} 
Alg.~\ref{alg:main} is implemented with $3000$ lines of Python code in 7 modules\footnote{\legos{} implementation is available in \hl{TODO: add link anonymous github}}. We use the PySMT~\cite{Gario-et-al-2015} library to formulate SMT queries and interface with our SMT back-end solver, z3~\cite{Leonardo-Nikolaj-2008}. We adopted MaxRes's maxsat algorithm~\cite{Narodytska-et-al-14} to compute the minimum solution during domain expansion. \legos{} also has a web GUI, for which the front-end is implemented with $1400$ lines of JavaScript code and the back-end with 76 lines of Python code. 
%As shown in Fig.~\ref{fig:web-gui}, the web GUI includes three editors where the user provides: (1) the domain of the system (i.e., user-define types), (2) the system requirements, and (3) the LP to check; and an option bar where the user can specify the volume and activate specific optimizations (i.e., restart, boundary case reduction, universal blocking). Additionally, the \legos{} GUI automatically generates macros from the user-defined domain to assist the user in writing the requirements and properties. 
\legos{}'s web interface is available in \url{http://legos1.herokuapp.com/}.
\end{comment}
%\blue{
% BE:
%number of lines: 76 Description: Flask server that takes request from Frontend, launch verification, and after this sends a result to the Frontend
%FE:
%number of lines: 68178, (total: 215 files, 66850 codes, 156 comments, 1172 blanks)
%Description: React server that sent a request to Backend launch verification and after this show a result to the user.Description of different components (features):
%The main part is tree compilers, which take the user’s input. There is a feature that automatically generates macros for the user. The second important part - is the options bar, users can choose options (volume, restart, boundary case reduction, universal blocking) and the launch button. There is a menu dropdown, that enables the ability to see different examples. And a page with contact information.}
\begin{comment}
\begin{figure}
    \centering
    \includegraphics[scale=0.3]{img/legos-interface.png}
    \caption{Our web application \legos.}
    \label{fig:web-gui}
\end{figure}
\end{comment}

==> archive/eval-wednesday.tex <==
\section{Evaluation}
\label{sec:evaluation}
%Diagnosis consist in two part, proof based diag and API, while prroof are ..., we would like to be able to encapsulated in backend, to be able ro communicate to end usert langauge, 

%\hl{Proof and diagnosis Modular Theories}

In this section, we first evaluate the efficiency of \approach in generating proofs of unsatisfiability, its effectiveness in trimming the proof, and the utility of its \tfol diagnosis. 
%Our experiments aims to address two primary research questions:
% Effectiveness of LEGOS-PROOF
%subsection{Effectiveness of \approach}
Specifically, we aim to answer:  
\textbf{RQ1:} 
How efficient is the proof framework for generating proof in terms of time overhead? 
We utilize \approach to generate proofs, verify them, and measure the overhead associated with both proof generation and proof verification (employing a backward-checking mode).
Then, we aim to answer \textbf{RQ2:} How effective is \approach for trimming the proof? 
We  compare the initial size of the proof file and the number of derivation steps, with the ones trimmed.
Finally, we aim to answer: \textbf{RQ3:} How well does the instantiated diagnosis assist users in debugging identified inconsistencies? Through answering this question, we aim to determine whether the instantiated diagnosis provides meaningful insights for debugging inconsistencies. This demonstrate the utility of the \tfol diagnosis on a use case.   {\bf MC:  technique vs tool}
\approach implementation and the evaluation artifacts are available in \hl{TODO-Link}. 


\boldparagraph{Case studies}
We considered the \tfol requirements developed for eight real-world case-studies.
taken from the RESERVE repository of normative requirements~\cite{feng-et-al-24,feng-et-al-24b}: 
%\hl{TODO:  Put this in a table.}
(1) ALMI~\cite{Hamilton-et-al-22}: a system assisting elderly or disabled users in a monitoring/advisory role and with everyday tasks; 
(2) ASPEN~\cite{aspen-23}: an autonomous agent dedicated to forest protection, providing both diagnosis and treatment of various tree diseases; 
(3) AutoCar~\cite{autocar-20}: a system that implements emergency-vehicle priority awareness for autonomous vehicles; 
%(4) BSN~\cite{Gil-et-al-21}: a healthcare system detecting emergencies by continuously monitoring the patient’s health status; 
%(4) DressAssist~\cite{Jevtic-et-al-19,townsend-et-al-2022}: an assistive and supportive system used to dress and provide basic care for those in need; 
(4) CSI-Cobot~\cite{Stefanakos-et-al-22}: a system ensuring the safe integration of industrial collaborative robot manipulators; 
(5) DAISY~\cite{daisy-22}: a sociotechnical AI-supported system that directs patients through an A\&E triage pathway (our running example); 
%(6) DPA~\cite{Amaral-et-al-22}: a system to check  compliance of data processing agreements against the General Data Protection Regulation; 
(6) SafeSCAD~\cite{calinescu2021maintaining}: a driver attentiveness management system to support safe shared control of autonomous vehicles.
(7) Tabiat~\cite{tabiat}, a smartphone application (and sensors) that records symptoms and keeps doctors updated on patients' chronic obstructive pulmonary disease conditions; and (8) Casper~\cite{Moro-et-al-18}, a socially assistive robot designed to help people living with dementia by supporting activities of daily living at home and improving their quality of life.
% raison to select the case-studies
We have selected these case studies because they have been used in existing work~\cite{feng-et-al-24} which applied \tfol satisfiability to check well-formedness properties. Our goal is to use these case studies to evaluate the usability of the proofs generated by \approach.


\boldparagraph{Well-formedness properties}
\tfol has been used as an underlying formal language for SLEEC, a rule-based language for expressing normative requirements~\cite{Getir-Yaman-et-al-23}. 
The following well-formedness properties of SLEEC rules can be verified via \tfol unsatisfiability checking~\cite{feng-et-al-24}: \emph{vacuous conflict}, \emph{situational conflict}, \emph{redundancy}, and \emph{over-restrictiveness}. (i) a rule is  \emph{vacuously conflicting in a rule set $R$} if triggering this rule always leads to a conflict with some other rules in $R$; (ii) a rule is \emph{situationally conflicting in a rule set $R$} if triggering this rule under a certain situation, which defines a history of events and measures, always leads to a conflict with some other rules in the future; (iii) a rule is  \emph{redundant in a rule set $R$} if this rule is logically implied by other rules in $R$; and (vi) a rule set $R$ is \emph{overly restrictive subject to a given purpose} if none of the functional goals represented by the purpose is realizable while respecting $R$.
 Refer to \cite{feng-et-al-24} for formal definitions.
%\hl{TODO: introduce here each WFI - and diags.}


\boldparagraph{RQ1}
To answer RQ1, for each case study and well-formedness properties, we measure the overhead (time) of generating and checking the UNSAT proof for the existence of the well-formedness issues. The results are shown in Tbl.~\ref{tab:efficiency}. 
\nf{In total for the eight case-studies, we found 52 unsatisfiable instances. 
The average overhead was} \hl{X} \nf{seconds (with geometric mean} \hl{Y}\nf{\% ) and the maximum overhead was 2.5 seconds (Z\%).} 
%except for the SafeSCAD situational conflict instance which took approximately 2.5 seconds {\bf MC: ??}. 
For the 52 instances the overhead is sufficiently small, effectively addressing RQ1.



\boldparagraph{RQ2}
To answer RQ2, for each case study and well-formedness property, we measure the initial proof  size with the number of proof derivation steps, as well as the proof size and the number of steps remaining once trimmed (after checking the proof). The results are shown in the Tbl.~\ref{tab:effectiveness}. 
\hl{answer coming.}

\begin{table}[t]
    \centering
    \caption{Efficiency of generating UNSAT proofs. 
    For each generated UNSAT proof of well-formedness property, we record the time overhead  for generating and checking the proof. Significant overhead is in bold.}
    \label{tab:efficiency}
    \begin{tabular}{c c}
        \scalebox{0.8}{
            \begin{tabular}{r c c c c}
            \toprule
              case studies & \multicolumn{4}{c}{well-formedness}\\\cmidrule{2-5}
                & conflict & \multicolumn{1}{c}{s-conflict} & \multicolumn{1}{c}{redundancy} & \multicolumn{1}{c}{restrictiveness}\\
            \toprule
                        % ALMI ------------
                ALMI & \multicolumn{1}{c}{satisfiable} & 0.13 & \multicolumn{1}{c}{satisfiable}  & \multicolumn{1}{c}{satisfiable} \\\midrule
                % ASPEN ------------
                  ASPEN &\multicolumn{1}{c}{satisfiable} & 0.26 & 0.08 & \multicolumn{1}{c}{satisfiable}\\
                 %----
                  &\multicolumn{1}{c}{~} & 0.21 & & \multicolumn{1}{c}{~}\\
                 %----
                  &\multicolumn{1}{c}{~} & -0.05 & & \multicolumn{1}{c}{~}\\\midrule
                % Autocar ------------
                 AutoCar & \multicolumn{1}{c}{satisfiable} & \multicolumn{1}{c}{satisfiable} & 0.21 & \multicolumn{1}{c}{satisfiable}\\
                 %---
                 & \multicolumn{1}{c}{~} & \multicolumn{1}{c}{~} & 0.21 & \multicolumn{1}{c}{~}\\\midrule
                 %BSN & \multicolumn{5}{c}{satisfiable} &~& \multicolumn{5}{c}{satisfiable} &~& o & s & ss & s & ss &~& o & s & ss & s & ss\\
                 % Casper ------------
                 Casper & \multicolumn{1}{c}{satisfiable} & \multicolumn{1}{c}{satisfiable} & 0.17 & \multicolumn{1}{c}{satisfiable}\\\midrule 
                 % Tabiat --------------
                 Tabiat & -0.07 & 0.13 & 0.09 & 0.09\\
                 %--
                 & 0.05 & 0.13 & 0.09 & 0.1 \\
                 %--
                 & -0.04 & 0.13 & 0.13 & 0.11 \\
                 %--
                 & 0.03 & 0.14 & 0.12 &  \\
                 %--
                 & 0.01 & 0.13 & 0.09 &  \\
                 %--
                 & -0.16 & 0.14 &  & \\
                 %--
                 &  & 0.14 &  &   \\
                 %--
                 & & 0.13 &  &  \\
                 %--
                 &  & -0.19 & & \\
                 % DPA ------------
                 %DPA &  \multicolumn{5}{c}{satisfiable} &~& o & s & ss & s & ss &~& o & s & ss & s & ss &~& o & s & ss & s & ss\\ 
            \bottomrule
            \end{tabular}
        }
      &      
            \scalebox{0.8}{
            \begin{tabular}{r c c c c}
            \toprule
              case studies & \multicolumn{4}{c}{well-formedness}\\\cmidrule{2-5}
                & conflict & \multicolumn{1}{c}{s-conflict} & \multicolumn{1}{c}{redundancy} & \multicolumn{1}{c}{restrictiveness}\\
            \toprule
                % SafeSCAD ------------
                 SafeSCAD &  \multicolumn{1}{c}{satisfiable}  & 0.25 & 0.02 & 0.04\\
                 %--
                 &  \multicolumn{1}{c}{~}  & 0.22 & 0.02 & 0.03 \\
                 %--
                 &  \multicolumn{1}{c}{~}  & 0.23 &  &  \\
                 %--
                 &  \multicolumn{1}{c}{~}  & \textbf{2.25} &  &  \\
                 %--
                 &  \multicolumn{1}{c}{~}  & 0.34  &  &  \\
                 %--
                 &  \multicolumn{1}{c}{~}  & 0.26  &  &  \\
                 %--
                 &  \multicolumn{1}{c}{~}  & 0.29  &  &  \\
                 %--
                 &  \multicolumn{1}{c}{~}  & 0.27  &  &  \\
                 %--
                 &  \multicolumn{1}{c}{~}  & 0.32  &  &  \\
                 %--
                 &  \multicolumn{1}{c}{~}  & 0.56  &  &   \\
                 %--
                 &  \multicolumn{1}{c}{~}  & 0.33  &  &  \\\midrule
                % CSI ------------
                 CSI-Cobot & \multicolumn{1}{c}{satisfiable} & \multicolumn{1}{c}{satisfiable} & 0.12 & \multicolumn{1}{c}{satisfiable}\\
                 %-- 
                 & \multicolumn{1}{c}{~} & \multicolumn{1}{c}{~} & 0.12 & \multicolumn{1}{c}{~}\\
                 & \multicolumn{1}{c}{~} & \multicolumn{1}{c}{~} & 0.13 & \multicolumn{1}{c}{~}\\\midrule  
                % DAISY ------------
                 DAISY &  \multicolumn{1}{c}{satisfiable}  & 0.33 & 0.15 & \multicolumn{1}{c}{satisfiable} \\
                 &  \multicolumn{1}{c}{~}  & 0.29 &  &  \\  
                 \\
            \bottomrule
            \end{tabular}
        }
    \end{tabular}
\end{table}


\begin{table}[t]
    \centering
    \caption{Effectiveness of \approach for triming UNSAT proofs. 
    For each generated UNSAT proof of well-formedness property, the initial (init.) proof file size in Kilobyte (size) with the number of proof derivation steps (n-steps), as well as the proof file size and the number of steps remaining after checking the proof (check.).
    %Volume differences between $\opt$ and $\noopt$ are bolded. 
    }
    \label{tab:effectiveness}
    % time without time with initial step, steps after checking, steps once minimized
    \scalebox{0.8}{
    \begin{tabular}{r cccc c cccc c cccc c cccc}
        \toprule
         & \multicolumn{19}{c}{well-formedness property}\\\cmidrule{2-20}
        & \multicolumn{4}{c}{conflict} & ~ & \multicolumn{4}{c}{s-conflict} && \multicolumn{4}{c}{redundancy} && \multicolumn{4}{c}{restrictiveness}\\%\cmidrule{2-5}\cmidrule{7-9}\cmidrule{9-12}\cmidrule{14-20}
         \multirow{2}{*}{case studies} & \multicolumn{2}{c}{initial} & \multicolumn{2}{c}{check.} & & \multicolumn{2}{c}{initial} & \multicolumn{2}{c}{check.} && \multicolumn{2}{c}{initial} & \multicolumn{2}{c}{check.} && \multicolumn{2}{c}{initial} & \multicolumn{2}{c}{check.}\\%\cmidrule{3-6}\cmidrule{9-12}\cmidrule{15-18}\cmidrule{21-24}
         &size & n-steps & size & n-steps & & size & n-steps &  size & n-steps & & size & n-steps &  size & n-steps & & size & n-steps &  size & n-steps \\
         \toprule 
            % ALMI ------------
            ALMI & \multicolumn{4}{c}{satisfiable} &~& 256 & 664 & 104 & 137 &~& \multicolumn{4}{c}{satisfiable}  &~& \multicolumn{4}{c}{satisfiable} \\\midrule
            % ASPEN ------------
              ASPEN &\multicolumn{4}{c}{satisfiable} &~& 392 & 1607 & 76 & 118 &~& 151 & 751 & 27 & 101 &~& \multicolumn{4}{c}{satisfiable}\\
             %----
              &\multicolumn{4}{c}{~} &~& 230 & 745 & 76 & 111 &~&  &  &  &  &~& \multicolumn{4}{c}{~}\\
             %----
              &\multicolumn{4}{c}{~} &~& 268 & 832 & 76 & 111 &~&  &  &  &  &~& \multicolumn{4}{c}{~}\\\midrule
            % Autocar ------------
             AutoCar & \multicolumn{4}{c}{satisfiable} &~&  \multicolumn{4}{c}{satisfiable} &~& 143 & 576 & 29 & 97 &~& \multicolumn{4}{c}{satisfiable}\\
             %---
             & \multicolumn{4}{c}{~} &~&  \multicolumn{4}{c}{~} &~& 159 & 673 & 29 & 97 &~& \multicolumn{4}{c}{~}\\\midrule
             %BSN & \multicolumn{5}{c}{satisfiable} &~& \multicolumn{5}{c}{satisfiable} &~& o & s & ss & s & ss &~& o & s & ss & s & ss\\
            % Casper ------------
             Casper & \multicolumn{4}{c}{satisfiable} &~& \multicolumn{4}{c}{satisfiable} &~& 85 & 320 & 23 & 94 &~& \multicolumn{4}{c}{satisfiable}\\\midrule 
            % CSI ------------
             CSI-Cobot & \multicolumn{4}{c}{satisfiable} &~& \multicolumn{4}{c}{satisfiable} &~& 34 & 131 & 88 & 51 &~& \multicolumn{4}{c}{satisfiable}\\
             %-- 
             & \multicolumn{4}{c}{~} &~& \multicolumn{4}{c}{~} &~& 35 & 131 & 9 & 51 &~& \multicolumn{4}{c}{~}\\
             & \multicolumn{4}{c}{~} &~& \multicolumn{4}{c}{~} &~& 52 & 228 & 97 & 53 &~& \multicolumn{4}{c}{~}\\\midrule  
            % DAISY ------------
             DAISY &  \multicolumn{4}{c}{satisfiable}  &~& 648 & 1854 & 118 & 122 &~& 48 & 136 & 7 & 30 &~& \multicolumn{4}{c}{satisfiable} \\
             &  \multicolumn{4}{c}{~}  &~& 520 & 1470 & 117 & 122 &~&  &  &  &  &~& \multicolumn{4}{c}{~} \\\midrule         
             % DPA ------------
             %DPA &  \multicolumn{5}{c}{satisfiable} &~& o & s & ss & s & ss &~& o & s & ss & s & ss &~& o & s & ss & s & ss\\ 
            % SafeSCAD ------------
             SafeSCAD &  \multicolumn{4}{c}{satisfiable}  &~& 234 & 648 & 74 & 116 &~& 39 & 155 & 9 & 51 &~& 43 & 162 & 10 & 53\\
             %--
             &  \multicolumn{4}{c}{~}  &~&  240 & 779 & 68 & 67 &~& 40 & 159 & 10 & 53 &~& 42 & 169 & 10 & 60\\
             %--
             &  \multicolumn{4}{c}{~}  &~&  226 & 721 & 67 & 81 &~&  &  &  &  &~&  & & &\\
             %--
             &  \multicolumn{4}{c}{~}  &~&  244 & 843 & 88 & 162 &~&  &  &  &  &~&  & & &\\
             %--
             &  \multicolumn{4}{c}{~}  &~&  358 & 1175 & 100 & 204 &~&  &  &  &  &~&  & & &\\
             %--
             &  \multicolumn{4}{c}{~}  &~&  196 & 544 & 83 & 156 &~&  &  &  &  &~&  & & &\\
             %-- 
             &  \multicolumn{4}{c}{~}  &~&  236 & 793 & 88 & 162 &~&  &  &  &  &~&  & & &\\
             %--
             &  \multicolumn{4}{c}{~}  &~&  197 & 544 & 89 & 162 &~&  &  &  &  &~&  & & &\\
             %--
             &  \multicolumn{4}{c}{~}  &~&  248 & 674 & 101 & 207 &~&  &  &  &  &~&  & & &\\
             %--
             &  \multicolumn{4}{c}{~}  &~&  245 & 849 & 83 & 156 &~&  &  &  &  &~&  & & & \\
             %--
             &  \multicolumn{4}{c}{~}  &~&  263 & 769 & 101 & 207 &~&  &  &  &  &~&  & & &\\\midrule
             % Tabiat --------------
             Tabiat & 230 & 963 & 18 & 93 &~& 203 & 555 & 79 & 55 &~& 216 & 895 & 19 & 93 &~& 141 & 455 & 21 & 85\\
             %--
             & 133 & 398 & 18 & 73 &~& 232 & 586 & 71 & 34 &~& 50 & 165 & 9 & 44 &~& 236 & 1022 & 18 & 93\\
             %--
             & 256 & 1091 & 22 & 114 &~& 229 & 632 & 68 & 42 &~& 259 & 1089 & 14 & 73 &~& 237 & 1022 & 18 & 93\\
             %--
             & 233 & 963 & 18 & 93 &~& 199 & 542 & 90 & 105 &~& 231 & 945 & 19 & 93 &~&  &  &  & \\
             %--
             & 245 & 1028 & 18 & 93 &~& 200 & 542 & 91 & 105 &~& 233 & 947 & 19 & 93 &~&  &  &  &\\
             %--
             & 234 & 963 & 18 & 93 &~& 199 & 542 & 84 & 98 &~&    &  &  &  &~&   &  &  &\\
             %--
             &   & &  & &~& 244 & 657 & 85 & 93 &~&   &  &  &  &~&    &  &  &\\
             %--
             &   & &  & &~ & 257 & 699 & 69 & 34 &~&   &  &  &  &~&   &  &  &\\
             %--
             &  & &  & &~& 369 & 990 & 98 & 127 &~& &  &  &  &~&  &  &  &\\
        \bottomrule
    \end{tabular}
    }
    %\vspace{-0.2in}
\end{table}


% USABILITY of LEGOS-PROOD

\boldparagraph{RQ3}
%\boldparagraph{Models and Methods}
To answer RQ3, we conducted an experiment with five non-technical stakeholders (N-TSs) to determine whether the diagnoses obtained for eight RESERVE real-world case-studies %by leveraging the \tfol proof 
aids in understanding and resolving the specification inconsistencies.
The N-TSs included an ethicist, a lawyer, a philosopher, a psychologist, and a medical doctor.   {\bf MC:  END}
For different well-formedness properties, different diagnoses are generated. 
Therefore, for each property type, we measure how the information provided has been used by the N-TSs to resolve the WFIs:
(a) for vacuous conflict,redundancy and restrictiveness: the rules, events, and measures identified; and (b) for situational conflict: the rules and the events, measures in both the rules and the situation.
%for vacuous conflict and redundancy, the conflicting/redundant rules are identified with conflicting/redundant clause highlighted. 
%While for situational conflict and restrictiveness, a situation  %he to measure how the diagnosis helped the N-TS
%\hl{TODO: add metrics per WFI}

% Size of fragment: relevant info size extracted
% How much are highlight + how many clauses are highlighted

% Table
% case-studies - WFI types 
%                C R I Rs
%        USED/IDconflict/red - USED/CLAUSES - EVENTS/MEASURES in I/Rs
%     or Did not understand

% v-c s-v re - insu - restr
% ID rules, Clauses. vs  ID rules, clauses, nb event trace, nb meausres
% nb event - nb measures - nb event 

\begin{table}[t]
    \centering
    \caption{Caption \hl{[Table size will be reduced.]}}
    \label{tab:my_label}
    \scalebox{0.7}{
        \begin{tabular}{rc cc cccc cc ccc ccc}
        \toprule
            % header
             \multirow{3}{*}{case studies} && \multicolumn{14}{c}{well-formedness issues}  \\
             & & \multicolumn{2}{c}{conflict} & \multicolumn{4}{c}{s-conflicts} & \multicolumn{2}{c}{redundancy} & \multicolumn{3}{c}{insufficiency} & & \multicolumn{2}{c}{restrictiveness}\\ 
             && nR - nRu & nC - nCu & nR - nRu & nC - nCu & nSE - nSEu & nSM - nSMu & nR - nRu & nC - nCu & nE - nEu & nSE - nSEu & nSM - nSMu & nE - nEu & nSE - nSEu & nSM - nSMu\\
             \toprule
             ALMI && \multicolumn{2}{c}{NA} & \hl{39} - nRu & nC - nCu & nSE - nSEu & nSM - nSMu & \multicolumn{2}{c}{NA} & \multicolumn{3}{c}{NA} & \multicolumn{3}{c}{NA}\\
             ASPEN && \multicolumn{2}{c}{NA} & 15 - nRu & nC - nCu & nSE - nSEu & nSM - nSMu & nR - nRu & nC - nCu & nE - nEu & nSE - nSEu & nSM - nSMu & \multicolumn{3}{c}{NA}\\
             AutoCar && \multicolumn{2}{c}{NA} & 19 - nRu & nC - nCu & nSE - nSEu & nSM - nSMu & nR - nRu & nC - nCu & nE - nEu & nSE - nSEu & nSM - nSMu & \multicolumn{3}{c}{NA} \\
             %BSN && \multicolumn{2}{c}{NA} & \multicolumn{4}{c}{NA} & \multicolumn{2}{c}{NA} & nE - nEu & nSE - nSEu & nSM - nSMu & \multicolumn{3}{c}{NA}\\
             Casper && 26 - nRu & nC - nCu & 26 - nRu & nC - nCu & nSE - nSEu & nSM - nSMu & nR - nRu & nC - nCu & nE - nEu & nSE - nSEu & nSM - nSMu & nE - nEu & nSE - nSEu & nSM - nSMu\\
             %DressAssist && \multicolumn{2}{c}{NA} & 31 - nRu & nC - nCu & nSE - nSEu & nSM - nSMu & \multicolumn{2}{c}{NA} & nE - nEu & nSE - nSEu & nSM - nSMu & \multicolumn{3}{c}{NA}\\
             CSI-Cobot && \multicolumn{2}{c}{NA} & \multicolumn{4}{c}{NA} & 20 - nRu & nC - nCu & nE - nEu & nSE - nSEu & nSM - nSMu & \multicolumn{3}{c}{NA}\\
             DAISY && \multicolumn{2}{c}{NA} & 26 - nRu & nC - nCu & nSE - nSEu & nSM - nSMu & nR - nRu & nC - nCu & nE - nEu & nSE - nSEu & nSM - nSMu & \multicolumn{3}{c}{NA}\\
             %DPA && \multicolumn{2}{c}{NA} &  \multicolumn{4}{c}{NA} & \multicolumn{2}{c}{NA} & nE - nEu & nSE - nSEu & nSM - nSMu & \multicolumn{3}{c}{NA}\\
             SafeSCAD && \multicolumn{2}{c}{NA} & 28 - nRu & nC - nCu & nSE - nSEu & nSM - nSMu & nR - nRu & nC - nCu & nE - nEu & nSE - nSEu & nSM - nSMu & nE - nEu & nSE - nSEu & nSM - nSMu\\
             Tabiat && 28 - nRu & nC - nCu & 28 - nRu & nC - nCu & nSE - nSEu & nSM - nSMu & nR - nRu & nC - nCu & nE - nEu & nSE - nSEu & nSM - nSMu & nE - nEu & nSE - nSEu & nSM - nSMu\\
            \bottomrule
        \end{tabular}
    }
\end{table}


%  Collect data with
% ALMI - 39 rules - 41 e - 15 me
% ASPEN 15 (25 − 18) 
% AutoCar 19 (36-26) 
% BSN 29 (33-31)
% CASPER  26 (38-14)
% DressAssist 31 (54-42)
% CSI 20 (23-11)  
% DAISY 26 (28-25) 
% DPA 26 (28-25) 
% SafeSCAD 28 (29-20) 
% Tabia 28 (37 - 18)


\boldparagraph{Summary}


\boldparagraph{Threats to validity}
- Evaluation is maybe tool specific
- Generic object proof object we get from FOL*, it is effectiveness depend on the application, we only picked one.

%RQ2: Can the proof offer meaningful insights? We conduct a case study with several participants from sleec to determine whether the UNSAT core and the minimized proof aid in pinpointing inconsistencies within the specification.

% ArXiVE
%\subsection{RQ0}
%RQ0: The correctness of the proof. Show that the proofs generated for the selected case-studies are correct using an assistant proof and proof the assumption using the solver.

%\subsection{RQ1}
%RQ1: How applicable the proof framework is in terms of performance? We use LEGOs to emit proof and checks the proof and report the overhead for proof generation and proof checking (using backward-checking mode)


%\subsection{RQ2}
%RQ2: the effect of backward-checking compare to forward checking. Report the status of the checking time using backward checking vs forward checking. Report the proof size (compare to the original proof size) after minimization with backward checking.


%\subsection{RQ3}
%RQ3: Does the proof provide valuable insight. Do case study with sleec people. See if the UNSAT core and the minimized proof helps them find inconsistent specification. 


==> archive/oldJune24tables.tex <==
\begin{table*}[t]
    \centering
    \caption{Efficiency of generating UNSAT proofs. 
    For each generated UNSAT proof of well-formedness property, we record the time overhead  for generating and checking the proof. Significant overhead is in bold.}
    \label{tab:efficiency}
    \begin{tabular}{c c}
        \scalebox{0.8}{
            \begin{tabular}{r c c c c}
            \toprule
              case studies & \multicolumn{4}{c}{well-formedness}\\\cmidrule{2-5}
                & conflict & \multicolumn{1}{c}{s-conflict} & \multicolumn{1}{c}{redundancy} & \multicolumn{1}{c}{restrictiveness}\\
            \toprule
                % ALMI ------------
                ALMI & \multicolumn{1}{c}{satisfiable} & 0.13 & \multicolumn{1}{c}{satisfiable}  & \multicolumn{1}{c}{satisfiable} \\\midrule
                % ASPEN ------------
                  ASPEN &\multicolumn{1}{c}{satisfiable} & 0.26 & 0.08 & \multicolumn{1}{c}{satisfiable}\\
                 %----
                  &\multicolumn{1}{c}{~} & 0.21 & & \multicolumn{1}{c}{~}\\
                 %----
                  &\multicolumn{1}{c}{~} & -0.05 & & \multicolumn{1}{c}{~}\\\midrule
                % Autocar ------------
                 AutoCar & \multicolumn{1}{c}{satisfiable} & \multicolumn{1}{c}{satisfiable} & 0.21 & \multicolumn{1}{c}{satisfiable}\\
                 %---
                 & \multicolumn{1}{c}{~} & \multicolumn{1}{c}{~} & 0.21 & \multicolumn{1}{c}{~}\\\midrule
                 %BSN & \multicolumn{5}{c}{satisfiable} &~& \multicolumn{5}{c}{satisfiable} &~& o & s & ss & s & ss &~& o & s & ss & s & ss\\
                 % Casper ------------
                 Casper & \multicolumn{1}{c}{satisfiable} & \multicolumn{1}{c}{satisfiable} & 0.17 & \multicolumn{1}{c}{satisfiable}\\\midrule 
                 % Tabiat --------------
                 Tabiat & -0.07 & 0.13 & 0.09 & 0.09\\
                 %--
                 & 0.05 & 0.13 & 0.09 & 0.1 \\
                 %--
                 & -0.04 & 0.13 & 0.13 & 0.11 \\
                 %--
                 & 0.03 & 0.14 & 0.12 &  \\
                 %--
                 & 0.01 & 0.13 & 0.09 &  \\
                 %--
                 & -0.16 & 0.14 &  & \\
                 %--
                 &  & 0.14 &  &   \\
                 %--
                 & & 0.13 &  &  \\
                 %--
                 &  & -0.19 & & \\
                 % DPA ------------
                 %DPA &  \multicolumn{5}{c}{satisfiable} &~& o & s & ss & s & ss &~& o & s & ss & s & ss &~& o & s & ss & s & ss\\ 
            \bottomrule
            \end{tabular}
        }
      &      
            \scalebox{0.8}{
            \begin{tabular}{r c c c c}
            \toprule
              case studies & \multicolumn{4}{c}{well-formedness}\\\cmidrule{2-5}
                & conflict & \multicolumn{1}{c}{s-conflict} & \multicolumn{1}{c}{redundancy} & \multicolumn{1}{c}{restrictiveness}\\
            \toprule
                % SafeSCAD ------------
                 SafeSCAD &  \multicolumn{1}{c}{satisfiable}  & 0.25 & 0.02 & 0.04\\
                 %--
                 &  \multicolumn{1}{c}{~}  & 0.22 & 0.02 & 0.03 \\
                 %--
                 &  \multicolumn{1}{c}{~}  & 0.23 &  &  \\
                 %--
                 &  \multicolumn{1}{c}{~}  & \textbf{2.25} &  &  \\
                 %--
                 &  \multicolumn{1}{c}{~}  & 0.34  &  &  \\
                 %--
                 &  \multicolumn{1}{c}{~}  & 0.26  &  &  \\
                 %--
                 &  \multicolumn{1}{c}{~}  & 0.29  &  &  \\
                 %--
                 &  \multicolumn{1}{c}{~}  & 0.27  &  &  \\
                 %--
                 &  \multicolumn{1}{c}{~}  & 0.32  &  &  \\
                 %--
                 &  \multicolumn{1}{c}{~}  & 0.56  &  &   \\
                 %--
                 &  \multicolumn{1}{c}{~}  & 0.33  &  &  \\\midrule
                % CSI ------------
                 CSI-Cobot & \multicolumn{1}{c}{satisfiable} & \multicolumn{1}{c}{satisfiable} & 0.12 & \multicolumn{1}{c}{satisfiable}\\
                 %-- 
                 & \multicolumn{1}{c}{~} & \multicolumn{1}{c}{~} & 0.12 & \multicolumn{1}{c}{~}\\
                 & \multicolumn{1}{c}{~} & \multicolumn{1}{c}{~} & 0.13 & \multicolumn{1}{c}{~}\\\midrule  
                % DAISY ------------
                 DAISY &  \multicolumn{1}{c}{satisfiable}  & 0.33 & 0.15 & \multicolumn{1}{c}{satisfiable} \\
                 &  \multicolumn{1}{c}{~}  & 0.29 &  &  \\  
                 \\
            \bottomrule
            \end{tabular}
        }
    \end{tabular}
\end{table*}








%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{table*}[t]
    \centering
    \caption{Effectiveness of \approach for triming UNSAT proofs. 
    For each generated UNSAT proof of well-formedness property, the initial (init.) proof file size in Kilobyte (size) with the number of proof derivation steps (n-steps), as well as the proof file size and the number of steps remaining after checking the proof (check.).
    %Volume differences between $\opt$ and $\noopt$ are bolded. 
    }
    \label{tab:effectiveness}
    % time without time with initial step, steps after checking, steps once minimized
    \scalebox{0.8}{
    \begin{tabular}{r cccc c cccc c cccc c cccc}
        \toprule
         & \multicolumn{19}{c}{well-formedness property}\\\cmidrule{2-20}
        & \multicolumn{4}{c}{conflict} & ~ & \multicolumn{4}{c}{s-conflict} && \multicolumn{4}{c}{redundancy} && \multicolumn{4}{c}{restrictiveness}\\%\cmidrule{2-5}\cmidrule{7-9}\cmidrule{9-12}\cmidrule{14-20}
         \multirow{2}{*}{case studies} & \multicolumn{2}{c}{initial} & \multicolumn{2}{c}{check.} & & \multicolumn{2}{c}{initial} & \multicolumn{2}{c}{check.} && \multicolumn{2}{c}{initial} & \multicolumn{2}{c}{check.} && \multicolumn{2}{c}{initial} & \multicolumn{2}{c}{check.}\\%\cmidrule{3-6}\cmidrule{9-12}\cmidrule{15-18}\cmidrule{21-24}
         &size & n-steps & size & n-steps & & size & n-steps &  size & n-steps & & size & n-steps &  size & n-steps & & size & n-steps &  size & n-steps \\
         \toprule 
            % ALMI ------------
            ALMI & \multicolumn{4}{c}{satisfiable} &~& 104/256 & 137/664 & 104 & 137 &~& \multicolumn{4}{c}{satisfiable}  &~& \multicolumn{4}{c}{satisfiable} \\\midrule
            % ASPEN ------------
              ASPEN &\multicolumn{4}{c}{satisfiable} &~& 76/392 & 118/1607 & 76 & 118 &~& 27/151 & 101/751 & 27 & 101 &~& \multicolumn{4}{c}{satisfiable}\\
             %----
              &\multicolumn{4}{c}{~} &~& 76/230 & 111/745 & 76 & 111 &~&  &  &  &  &~& \multicolumn{4}{c}{~}\\
             %----
              &\multicolumn{4}{c}{~} &~& 76/268 & 111/832 & 76 & 111 &~&  &  &  &  &~& \multicolumn{4}{c}{~}\\\midrule
            % Autocar ------------
             AutoCar & \multicolumn{4}{c}{satisfiable} &~&  \multicolumn{4}{c}{satisfiable} &~& 29/143 & 97/576 & 29 & 97 &~& \multicolumn{4}{c}{satisfiable}\\
             %---
             & \multicolumn{4}{c}{~} &~&  \multicolumn{4}{c}{~} &~& 29/159 & 97/673 & 29 & 97 &~& \multicolumn{4}{c}{~}\\\midrule
             %BSN & \multicolumn{5}{c}{satisfiable} &~& \multicolumn{5}{c}{satisfiable} &~& o & s & ss & s & ss &~& o & s & ss & s & ss\\
            % Casper ------------
             Casper & \multicolumn{4}{c}{satisfiable} &~& \multicolumn{4}{c}{satisfiable} &~& 23/85 & 94/320 & 23 & 94 &~& \multicolumn{4}{c}{satisfiable}\\\midrule 
            % CSI ------------
             CSI-Cobot & \multicolumn{4}{c}{satisfiable} &~& \multicolumn{4}{c}{satisfiable} &~& 88/34 & 51/131 & 88 & 51 &~& \multicolumn{4}{c}{satisfiable}\\
             %-- 
             & \multicolumn{4}{c}{~} &~& \multicolumn{4}{c}{~} &~& 9/35 & 51/131 & 9 & 51 &~& \multicolumn{4}{c}{~}\\
             & \multicolumn{4}{c}{~} &~& \multicolumn{4}{c}{~} &~& 97/52 & 53/228 & 97 & 53 &~& \multicolumn{4}{c}{~}\\\midrule  
            % DAISY ------------
             DAISY &  \multicolumn{4}{c}{satisfiable}  &~& 118/648 & 122/1854 & 118 & 122 &~& 7/48 & 30/136 & 7 & 30 &~& \multicolumn{4}{c}{satisfiable} \\
             &  \multicolumn{4}{c}{~}  &~& 117/520 & 122/1470 & 117 & 122 &~&  &  &  &  &~& \multicolumn{4}{c}{~} \\\midrule         
             % DPA ------------
             %DPA &  \multicolumn{5}{c}{satisfiable} &~& o & s & ss & s & ss &~& o & s & ss & s & ss &~& o & s & ss & s & ss\\ 
            % SafeSCAD ------------
             SafeSCAD &  \multicolumn{4}{c}{satisfiable}  &~& 74/234 & 116/648 & 74 & 116 &~& 9/39 & 51/155 & 9 & 51 &~& 10/43 & 53/162 & 10 & 53\\
             %--
             &  \multicolumn{4}{c}{~}  &~& 68/240 & 67/779 & 68 & 67 &~& 10/40 & 53/159 & 10 & 53 &~& 10/42 & 60/169 & 10 & 60\\
             %--
             &  \multicolumn{4}{c}{~}  &~& 67/226 & 81/721 & 67 & 81 &~&  &  &  &  &~&  & & &\\
             %--
             &  \multicolumn{4}{c}{~}  &~&  88/244 & 162/843 & 88 & 162 &~&  &  &  &  &~&  & & &\\
             %--
             &  \multicolumn{4}{c}{~}  &~&  100/358 & 204/1175 & 100 & 204 &~&  &  &  &  &~&  & & &\\
             %--
             &  \multicolumn{4}{c}{~}  &~&  83/196 & 156/544 & 83 & 156 &~&  &  &  &  &~&  & & &\\
             %-- 
             &  \multicolumn{4}{c}{~}  &~&  88/236 & 162/793 & 88 & 162 &~&  &  &  &  &~&  & & &\\
             %--
             &  \multicolumn{4}{c}{~}  &~&  89/197 & 162/544 & 89 & 162 &~&  &  &  &  &~&  & & &\\
             %--
             &  \multicolumn{4}{c}{~}  &~&  101/248 & 207/674 & 101 & 207 &~&  &  &  &  &~&  & & &\\
             %--
             &  \multicolumn{4}{c}{~}  &~&  83/245 & 156/849 & 83 & 156 &~&  &  &  &  &~&  & & & \\
             %--
             &  \multicolumn{4}{c}{~}  &~&  101/263 & 207/769 & 101 & 207 &~&  &  &  &  &~&  & & &\\\midrule
             % Tabiat --------------
             Tabiat & 18/230 & 93/963 & 18 & 93 &~& 79/203 & 55/555 & 79 & 55 &~& 19/216 & 93/895 & 19 & 93 &~& 21/141 & 85/455 & 21 & 85\\
             %-- TODO HERE
             & 18/133 & 73/398 & 18 & 73 &~& 71/232 & 34/586 & 71 & 34 &~& 9/50 & 44/165 & 9 & 44 &~& 18/236 & 93/1022 & 18 & 93\\
             %--
             & 22/256 & 114/1091 & 22 & 114 &~& 68/229 & 42/632 & 68 & 42 &~& 15/259 & 73/1089 & 14 & 73 &~& 18/237 & 93/1022 & 18 & 93\\
             %--
             & 18/233 & 93/963 & 18 & 93 &~& 90/199 & 105/542 & 90 & 105 &~& 19/231 & 93/945 & 19 & 93 &~&  &  &  & \\
             %--
             & 18/245 & 93/1028 & 18 & 93 &~& 91/200 & 105/542 & 91 & 105 &~& 19/233 & 93/947 & 19 & 93 &~&  &  &  &\\
             %--
             & 18/234 & 93/963 & 18 & 93 &~& 84/199 & 98/542 & 84 & 98 &~&    &  &  &  &~&   &  &  &\\
             %--
             &   & &  & &~& 85/244 & 93/657 & 85 & 93 &~&   &  &  &  &~&    &  &  &\\
             %--
             &   & &  & &~ & 69/257 & 34/699 & 69 & 34 &~&   &  &  &  &~&   &  &  &\\
             %--
             &  & &  & &~& 98/369 & 127/990 & 98 & 127 &~& &  &  &  &~&  &  &  &\\
        \bottomrule
    \end{tabular}
    }
    %\vspace{-0.2in}
\end{table*}

==> archive/overview.tex <==
\boldparagraph{\blue{Tool support}}
%
%\hl{\textbf{TODO}: refer to figure 2 components, and update references}. 
\nf{We implemented our approach in a tool called \legos{} that takes as input \folstarplus{} formulas}\footnote{\nf{\legos{} uses \ibs{} translation component to also support MFOTL formulas.}}. 
\nf{\legos{} is build on top of \ibs{} tool with 1200 lines of Python code~\cite{tacas-supp}.} \hl{TODO udate github links.} \nf{We use the PySMT~\cite{Gario-et-al-2015} library to formulate SMT queries and interface with our SMT back-end solver, Z3~\cite{Leonardo-Nikolaj-2008}. We adopted MaxRes's maxsat algorithm~\cite{Narodytska-et-al-14} to compute the minimum solution during domain expansion. 
\legos{} also has a web interface (available in~\cite{tacas-tool}), implemented with $1400$ lines of JavaScript code in the front-end and about 100 lines of Python code in the back-end.} 
\nf{For \legos{} architecture see Sec.~\ref{ap:architecture}.}

%\blue{In this section, we describe an overview of our approach, \legos{}, that extends \ibs{} to solve the bounded satisfiability of \nf{\folstar{}} formulas with aggregation (\nf{\folstarplus}).} 
%\blue{\legos takes as input \nf{\folstarplus{}} requirements \textit{Reqs}, an \nf{\folstarplus{}} property $\phi$, and a volume bound $b_{vol}$. 
%It searches for a counterexample $\sigma$ bounded by $b_{vol}$ that satisfies the requirements \textit{Reqs} while violating the property $\phi$, i.e., $\phi \bigwedge_{\psi \in \textit{Reqs} \psi}$.  
%If no counterexample can be found regardless of the bound $b_{vol}$, \legos{} returns \unsat; otherwise, if a solution might exist given a larger bound, it returns \bunsat. }

%\legos{} extends \ibs{} components \textsc{Search} and \textsc{Ground} (see Sec.~\ref{sec:background}) with aggregation support (see Sec.~\ref{sec:aggregation}) \nf{and the four optimizations (see Sec.~\ref{sec:approach})}.  
%The architecture of \legos{} is   shown in Fig.~\ref{fig:architecture-c}.
% schema
%\input{fig-tool}


%\nf{The component \textsc{Search} looks for a solution to these formulas.} \textsc{Search} invokes the component \textsc{Ground} to produce grounded over- and under-approximation queries. The queries are then solved by an SMT solver in component \textsc{Solve}. Depending on the satisfiability results returned by \textsc{Solve}, \textsc{Search} either (1) terminates by returning a counterexample, \unsat{} or \bunsat, or (2) expands the search domain. After expanding the search domain, \textsc{Search} invokes \textsc{Ground} again to produce new approximation queries.


%\legos{} extends \ibs's components  \textsc{Search} and \textsc{Ground} to support aggregation.  In addition, component \textsc{Search} is extended with optimizations 
%\textit{relaxed domain expansion}, \textit{restart}, and \textit{incremental solving} (see below), and component
%\textsc{Ground} -- with the optimization \textit{boundary case reduction}. Other components, colored gray in Fig.~\ref{fig:architecture-c}, are directly reused from \ibs{}~\cite{Feng-et-al-22} and Z3~\cite{Leonardo-Nikolaj-2008}.
%

%We implemented \legos{} on top of \ibs{} with 1200 lines of Python code~\cite{tacas-supp}. We use the PySMT~\cite{Gario-et-al-2015} library to formulate SMT queries and interface with our SMT back-end solver, Z3~\cite{Leonardo-Nikolaj-2008}. 
%We adopted MaxRes's maxsat algorithm~\cite{Narodytska-et-al-14} to compute the minimum solution during domain expansion. 
%\legos{} also has a web interface (available in~\cite{tacas-tool}), implemented with
 %$1400$ lines of JavaScript code in the front-end and about 100 lines of Python code in the back-end.

==> archive/tableARc.tex <==
  \scalebox{0.8}{
        \begin{tabular}{r c c c c}
        \toprule
          case studies & \multicolumn{4}{c}{well-formedness}\\\cmidrule{2-5}
            & conflict & \multicolumn{1}{c}{s-conflict} & \multicolumn{1}{c}{redundancy} & \multicolumn{1}{c}{restrictiveness}\\
        \toprule
                    % ALMI ------------
            ALMI & \multicolumn{1}{c}{satisfiable} & 0.13 & \multicolumn{1}{c}{satisfiable}  & \multicolumn{1}{c}{satisfiable} \\\midrule
            % ASPEN ------------
              ASPEN &\multicolumn{1}{c}{satisfiable} & 0.26 & 0.08 & \multicolumn{1}{c}{satisfiable}\\
             %----
              &\multicolumn{1}{c}{~} & 0.21 & & \multicolumn{1}{c}{~}\\
             %----
              &\multicolumn{1}{c}{~} & -0.05 & & \multicolumn{1}{c}{~}\\\midrule
            % Autocar ------------
             AutoCar & \multicolumn{1}{c}{satisfiable} & \multicolumn{1}{c}{satisfiable} & 0.21 & \multicolumn{1}{c}{satisfiable}\\
             %---
             & \multicolumn{1}{c}{~} & \multicolumn{1}{c}{~} & 0.21 & \multicolumn{1}{c}{~}\\\midrule
             %BSN & \multicolumn{5}{c}{satisfiable} &~& \multicolumn{5}{c}{satisfiable} &~& o & s & ss & s & ss &~& o & s & ss & s & ss\\
            % Casper ------------
             Casper & \multicolumn{1}{c}{satisfiable} & \multicolumn{1}{c}{satisfiable} & 0.17 & \multicolumn{1}{c}{satisfiable}\\\midrule 
            % CSI ------------
             CSI-Cobot & \multicolumn{1}{c}{satisfiable} & \multicolumn{1}{c}{satisfiable} & 0.12 & \multicolumn{1}{c}{satisfiable}\\
             %-- 
             & \multicolumn{1}{c}{~} & \multicolumn{1}{c}{~} & 0.12 & \multicolumn{1}{c}{~}\\
             & \multicolumn{1}{c}{~} & \multicolumn{1}{c}{~} & 0.13 & \multicolumn{1}{c}{~}\\\midrule  
            % DAISY ------------
             DAISY &  \multicolumn{1}{c}{satisfiable}  & 0.33 & 0.15 & \multicolumn{1}{c}{satisfiable} \\
             &  \multicolumn{1}{c}{~}  & 0.29 &  &  \\\midrule         
             % DPA ------------
             %DPA &  \multicolumn{5}{c}{satisfiable} &~& o & s & ss & s & ss &~& o & s & ss & s & ss &~& o & s & ss & s & ss\\ 
            % SafeSCAD ------------
             SafeSCAD &  \multicolumn{1}{c}{satisfiable}  & 0.25 & 0.02 & 0.04\\
             %--
             &  \multicolumn{1}{c}{~}  & 0.22 & 0.02 & 0.03 \\
             %--
             &  \multicolumn{1}{c}{~}  & 0.23 &  &  \\
             %--
             &  \multicolumn{1}{c}{~}  & 2.25 &  &  \\
             %--
             &  \multicolumn{1}{c}{~}  & 0.34  &  &  \\
             %--
             &  \multicolumn{1}{c}{~}  & 0.26  &  &  \\
             %--
             &  \multicolumn{1}{c}{~}  & 0.29  &  &  \\
             %--
             &  \multicolumn{1}{c}{~}  & 0.27  &  &  \\
             %--
             &  \multicolumn{1}{c}{~}  & 0.32  &  &  \\
             %--
             &  \multicolumn{1}{c}{~}  & 0.56  &  &   \\
             %--
             &  \multicolumn{1}{c}{~}  & 0.33  &  &  \\\midrule
             % Tabiat --------------
             Tabiat & -0.07 & 0.13 & 0.09 & 0.09\\
             %--
             & 0.05 & 0.13 & 0.09 & 0.1 \\
             %--
             & -0.04 & 0.13 & 0.13 & 0.11 \\
             %--
             & 0.03 & 0.14 & 0.12 &  \\
             %--
             & 0.01 & 0.13 & 0.09 &  \\
             %--
             & -0.16 & 0.14 &  & \\
             %--
             &  & 0.14 &  &   \\
             %--
             & & 0.13 &  &  \\
             %--
             &  & -0.19 & & \\
        \bottomrule
        \end{tabular}
    }

==> diagnosis.tex <==
\section{Diagnosing SLEEC WFIs with \tfol}



==> overview.tex <==
\section{Proof Framework Modulo
 Theories}\label{sec:proofFramework}


% \hl{TODO: move earlier, and if needed add the background.}

% \hl{TODO: add theorems proof each properties, add a schema, make it stronger}

% \hl{TODO: generic proof rules, generic proof validation, and generic proof diagnosis, then parallelism, once we instantiate it wit FOL*.}

In this section, we present a general framework for Refutation Proof Modulo Theories (RPMT). This proof framework enables integration with external theory reasoning to assist in the derivation of UNSAT

Suppose $\mathbb{L}$, e.g., \tfol, is the target language to be supported for proof of UNSAT and $\mathbb{T}$ is an external theory (or a theory combination), e.g., LIA, for which a decision procedure exists. We assume that $\mathbb{T}$ and $\mathbb{L}$ intersect with consistent interpretation on \textit{at least} boolean logic symbols (i.e., $\top$, $\bot$, $\wedge$, $\neg$). 
Let a set of input constraints $\mathbb{L}$ be given as $R$. A proof of UNSAT for $R$ is a sequence of derivation steps $d_1, \ldots, d_n$ where every step $d_i$ is an application of one of the derivation rules that transforms the proof state $s_{i-1}$ into a new state $s_i$. A proof state $s_i = (R^+_i, F_i, \domain_i)$ consists of three elements:
\begin{itemize}
     \item Lemmas (denoted as $R^+_i$) is the set of formulas in $\mathbb{L}$ which have been proven, $R^+_0 \gets R$.
    \item Facts (denoted as $F_i$) is the set of formulas in $\mathbb{T}$,  $F_0 \gets \emptyset$.
    \item The side-effect objects (SEOs) (denoted as $D_i$), which are used to capture the side-effects of the derivations (e.g., names of the used variables). The initialization of $D_0$ depends on the type of SEOs.
\end{itemize}

% We assume that all lemmas, facts, and relational objects have a unique numerical ID and the function \textit{ID} returns the ID of a given rule, fact or relational object. 
% Moreover, each lemma $\phi$ has a  boolean definition variable $b_\phi$ such that $p_\phi = \top$ if and only if $\phi$ holds. We denote $\textit{DEF}(\phi) = b_\phi$. 

Each derivation step $d_i = (\textit{rule}, Dep_i, F_i^\Delta, R_i^\Delta, D_i^\Delta)$ consist of (1) \textit{rule}: the name of derivation rule being applied to, (2) $Dep_i = (R', F', D')$: sets of dependant lemmas $R'_i$, facts $F'_i$ and side-effect objects $\domain'_i$ that enables the derivation, (3) $F_i^\Delta$: new facts added by applying $d_i$, (4) $R_i^\Delta$: new lemmas derived by $d_i$, and (5) $D_i^\Delta$ new SEOs added by $d_i$. We say the dependencies is $Dep_i$ is \textit{satisfied} in state  $s_{i-1}$, denoted as $Dep_i \subseteq s_{i-1}$ if $R'_i \subseteq R^+_i$, $F'_i \subseteq F_{i-1}$, and $\domain'_i \subseteq \domain_{i-1}$.
Given a state $s_{i-1} = (F_{i-1}, R^+_{i-1}, D_{i-1})$, if $Dep_i \subseteq s_{i-1}$ 
 and the \textit{rule} specific enabling condition, denoted as $PC_{\textit{rule_i}}$ holds on $d_i$, then applying $d_i$ adds the newly derived resources in $ F_i^\Delta$, $R_i^\Delta$, and $D_i^\Delta$ to $F_{i-1}$, $R^+_{i-1}$, and $D_{i-1}$, respectively.

Formally, the application of $d_i = (\textit{rule}_i, Dep_i, F_i^\Delta, R_i^\Delta, D_i^\Delta)$ on the state $s_{i-1} = (F_{i-1}, R^+_{i-1}, D_{i-1})$, denoted as $s_{i-1}\circ d_i$, yields a new state $s_i = (F_{i}, R^+_{i}, D_{i})$ such that:
\[
 s_i = \begin{cases}
 \emptyset & \text{if } s_{i-1} = \emptyset \\
  (F_{i-1} \cup F_i^\Delta, R^+_{i-1} \cup R_i^\Delta, D_{i-1} \cup D_i^\Delta )  & \text{else if } Dep_i \subseteq s_{i-1} \wedge \textit{PC}_{rule_i}(d_i) \\
  \emptyset & \text{otherwise}
\end{cases}
\]
where $\emptyset$ is a dead-end state representing derivation error and function \textit{PC}$(rule_i, Dep_i)$ checks if the listed resources in $Dep_i$ is sufficient to satisfy the enabling condition specific to each \textit{rule}.  

The proof framework supports the following three meta derivation rules: (1) \textbf{$\mathbb{T}$-Derive} enables external reasoning in $\mathbb{T}$; (2) (\textbf{$\mathbb{L} \rightarrow \mathbb{T}$}) communicates from $\mathbb{L}$ lemmas in $R^+$ to $\mathbb{T}$ facts in $F$; and (3) \textbf{$\mathbb{T} \rightarrow \mathbb{L}$} communicates from $\mathbb{T}$ to $\mathbb{L}$. The communications between $\mathbb{L}$ and $\mathbb{T}$ are realized through the intersection of the two languages. Formally:
%The proof framework supports the following meta derivation rules to enables external reasoning in $\mathbb{T}$ (\textbf{$\mathbb{T}$-Derive}) and communication between $\mathbb{L}$ lemmas in $R^+$ and $\mathbb{T}$ facts in $F$ (\textbf{$\mathbb{L} \rightarrow \mathbb{T}$} and \textbf{$\mathbb{T} \rightarrow \mathbb{L}$}) via the intersection of $\mathbb{L}$ and $\mathbb{T}$:


 \textbf{(1) $\mathbb{T}$-Derive}: if there exists a subset of facts $F' \subseteq F$ such that $F'$ derives a new fact $\phi_g$ in $\mathbb{T}$ (i.e., $F' \models^{\mathbb{T}} \phi_g$) , then applying rule \textbf{$\mathbb{T}$-Derive} adds $\phi_g$ to $F_i$. The fact $\phi_g$ depends on $F'$, denoted as  $\dep{\phi_{g}} = F'$. Formally,
    \begin{definition}\label{rule:derive}
    Let a derivation step $d_i = (\textit{rule}_i, Dep_i, F_i^\Delta, R_i^\Delta, D_i^\Delta)$ and a formula $\phi_g$ in theory $\mathbb{T}$ be given where $Dep_i = (R'_i, F'_i, \domain'_i)$. The step $d_i$ is a valid application of \textbf{$\mathbb{T}$-Derive} rule if:
    \[
        PC_{\textbf{$\mathbb{T}$-Derive}}(d_i) := R^\Delta_i = \domain^\Delta_i = \emptyset \wedge F^\Delta_i = \{\phi_g\} \wedge F'_i \models^{\mathbb{T}} \phi_g
    \]    
        
    \end{definition}
    
    \textbf{(2) $\mathbb{L} \rightarrow \mathbb{T}$}: If a $\mathbb{L}$ lemma $\phi \in R^+$ is in the intersection of $\mathbb{L}$ and $\mathbb{T}$, then $\phi$ can be added to $F$ as a $\mathbb{T}$ fact. Formally:
     \begin{definition}\label{rule:LtoT}
    Let a derivation step $d_i = (\textit{rule}_i, Dep_i, F_i^\Delta, R_i^\Delta, D_i^\Delta)$ and a $\mathbb{L}$ formula $\phi$ in be given where $ Dep_i := (R'_i, F'_i, \domain'_i)$. The step $d_i$ is a valid application of \textbf{$\mathbb{L} \rightarrow \mathbb{T}$} rule if:
    \[
         PC_{\textbf{$\mathbb{L} \rightarrow \mathbb{T}$}}(d_i) := R^\Delta_i = \domain^\Delta_i = \emptyset \wedge F^\Delta_i = \{\phi\} \wedge \phi \in R'_i \wedge \phi \in \mathbb{T}
    \]    
        
    \end{definition}
    \textbf{(3) $\mathbb{T} \rightarrow \mathbb{L}$:} If a $\mathbb{T}$ fact $\phi \in F$ is in the intersection of $\mathbb{L}$ and $\mathbb{T}$, then $\phi$ can be added to $R^+$ as a $\mathbb{L}$ lemma.
    \begin{definition}\label{rule:TtoL}
    Let a derivation step $d_i = (\textit{rule}_i, Dep_i, F_i^\Delta, R_i^\Delta, D_i^\Delta)$ and a $\mathbb{T}$ formula $\phi$ in be given where $ Dep_i := (R'_i, F'_i, \domain'_i)$. The step $d_i$ is a valid application of \textbf{$\mathbb{L} \rightarrow \mathbb{T}$} rule if: 
    \[
         PC_{\textbf{$\mathbb{T} \rightarrow \mathbb{L}$}}(d_i) := F^\Delta_i = \domain^\Delta_i = \emptyset \wedge R^\Delta_i = \{\phi\} \wedge \phi \in F'_i \wedge \phi \in \mathbb{L}
    \]           
    \end{definition}
 

Since $\mathbb{L}$ and $\mathbb{T}$ intersect on boolean logic, the communication between $\mathbb{L}$ and $\mathbb{T}$ is always possible.   

\begin{remark}
    We can extend the RPMT framework to work with a set of external theories $\mathbb{TS}$ that intersect on boolean logic. The resulting framework simulates the reasoning steps of DPLL(T) framework where $\mathbb{L}$ is the union of all used first-order theories and every $\mathbb{T} \in \mathbb{TS}$ is an individual theory in the union. The communication between $\mathbb{L}$ and  $\mathbb{T}$ are carried out via boolean abstraction.
\end{remark}

==> table.tex <==

    \begin{table}[t]
        \centering
        \scalebox{0.75}{
        \begin{tabular}{|c c| |c|c|c| |c|c|c|}
            \toprule
            \multicolumn{2}{|c||}{case studies} & \multicolumn{3}{|c||}{\legos} & \multicolumn{3}{|c|}{\ibs} \\ \cline{3-8}
            & & res. & time & mem. & res. & time & mem. \\\toprule
            \multirow{3}{*}{BST} & $bs_1$ & \unsat & 0.44 & 88 & \unsat & 0.50 & 89\\
             & $bs_2$ & 2 & 0.22 & \colorbox{orange!20}{63} & 2 & 0.21 & \colorbox{blue!20}{32}\\
             & $bs_3$ & 5 & 0.46 & 89 & 5 & 0.95 & 92\\\toprule
            % config 1
            \multirow{12}{*}{NASA} & $na_1$ & \unsat & 1.11 & \colorbox{orange!20}{172} & \unsat & 1.17 & \colorbox{blue!20}{108}\\
             & $na_2$ & \unsat & 0.42 & \colorbox{orange!10}{161} & \unsat & 0.38 & \colorbox{blue!10}{96}\\
             & $na_3$ & \unsat & 0.42 & \colorbox{orange!10}{162} & \unsat & 0.35 & \colorbox{blue!10}{96}\\
             & $na_4$ & \unsat & 1.14 & 99 & \unsat & 1.15 & 100\\
             & $na_5$ & \unsat & 0.32 & \colorbox{orange!10}{159} & \unsat & 0.29 & \colorbox{blue!10}{95}\\
             & $na_6$ & \unsat & 0.21 & 61 & \unsat & 0.20 & 60\\ 
             % config 2
             & $na_{1b}$ & \unsat & 0.36 & \colorbox{orange!10}{161} & \unsat & 0.31 & \colorbox{blue!10}{92}\\
             & $na_{2b}$ & \unsat & 0.36 & \colorbox{orange!10}{161} & \unsat & 0.32 & \colorbox{blue!10}{92}\\
             & $na_{3b}$ & \unsat & 0.36 & \colorbox{orange!10}{161} & \unsat & 0.31 & \colorbox{blue!10}{96}\\
             & $na_{4b}$ & \unsat & 0.39 & 88 & \unsat & 0.33 & 89\\
             & $na_{5b}$ & \unsat & 0.37 & \colorbox{orange!10}{161} & \unsat & 0.33 & \colorbox{blue!10}{92}\\
             & $na_{6b}$ & \unsat & 0.20 & 62 & \unsat & 0.21 & 60\\
            \bottomrule
        \end{tabular}
        } % 
        \scalebox{0.75}{
        \begin{tabular}{|c c| |c|c|c| |c|c|c|}
            \toprule
            \multicolumn{2}{|c||}{case studies} & \multicolumn{3}{|c||}{\legos} & \multicolumn{3}{|c|}{\ibs} \\ \cline{3-8}
            & & res. & time & mem. & res. & time & mem. \\\toprule
            \multirow{7}{*}{CF@H} & $cf_1$ & \unsat & 1.56 & 100 & \unsat & 1.51 & 95\\
             & $cf_2$ & 14 & \colorbox{green!10}{2.17} & 101 & 14 & \colorbox{red!10}{6.79} & 120\\
             & $cf_3$ & 16 & \colorbox{green!20}{3.04} & 103 & 16 & \colorbox{red!20}{13.73} & 138\\
             & $cf_4$ & 14 & \colorbox{green!30}{4.36} & \colorbox{blue!30}{116} & 14 & \colorbox{red!30}{71.42} & \colorbox{orange!30}{309}\\
             & $cf_5$ & 8 & 0.74 & 88 & 8 & 0.89 & 89\\
             & $cf_6$ & 8 & 0.61 & 88 & 8 & 0.90 & 90\\
             & $cf_7$ & \unsat & 0.41 & 86 & \unsat & 0.82 & 91\\ \toprule
            PBC & $pb_1$ & 9 & 0.52 & 87 & 9 & 0.52 & 87\\ \toprule 
            \multirow{7}{*}{PHIM} & $ph_1$ & \unsat & 0.21 & 80 & \unsat & 0.20 & 32\\
             & $ph_2$ & \unsat & 0.18 & 80 & \unsat & 0.21 & 59\\
             & $ph_3$ & \unsat & 0.23 & 69 & \unsat & 0.21 & 59\\
             & $ph_4$ & \unsat & 0.21 & 61 & \unsat & 0.21 & 59\\
             & $ph_5$ & 56 & \colorbox{green!10}{19.78} & \colorbox{blue!20}{308} & 56 & \colorbox{red!20}{32.92} & \colorbox{orange!20}{407}\\
             & $ph_6$ & \unsat & 0.87 & 92 & \unsat & 1.12 & 92\\
             & $ph_7$ & 19 & \highlightw{black}{\colorbox{green!30}{\textbf{10.54}}} & \colorbox{blue!30}{\textbf{136}} & 19 & \colorbox{red!30}{322} & \colorbox{orange!30}{253}\\
            \bottomrule
        \end{tabular}
        } % 
        \caption{{\footnotesize Run-time performance of \legos{} and \ibs{} for five case-studies and their properties.   We report  result (res.), running time (time, in seconds) and memory (mem., in MB). Darker orange represents a larger memory footprint and blue---a lower one. Darker red represents a longer execution time, and darker green---a faster one.}}
        \label{tab:eval-results}
    \vspace{-0.20in}
    \end{table}
%----
%\begin{minipage}{17em}
\begin{table}[t]
    %\centering
    %------------------------ Table 1
        \scalebox{0.75}{
    \begin{tabular}{|c c||c|c|c|c|c|}
    \toprule 
    \multicolumn{2}{|c||}{case studies} & res. & no opt & bcr & %\multicolumn{2}{|c||}{ub} &
    restart & all
    \\ %\toprule 
    \cline{4-5}\cline{6-6}\cline{7-7}
    & & & time & time & time & time \\ \toprule
    %-----------
    
    %-----------
    \multirow{5}{*}{DGraph} & 
    $dg1$ & 10 & {24.4} & {24.5} & \colorbox{red!20}{64.2} & {17.1} \\
    & $dg2$ & 12&   \colorbox{red!30}{916.1} & 122.3 & 176 & \colorbox{green!20}{ 65.8 } \\
    %& $dg4$ & o & \multicolumn{2}{|c||}{\colorbox{red!30}{timeout}} &   t & m &   t & m &   t & m &   t & m  \\
    %& $dg5$ & o &  t & m &   t & m &  t & m &   t & m  \\
    %& $dg6$ & o &  t & m &   t & m & t & m &  t & m  \\
    & $dg3$ & 10 & \colorbox{red!10}{46.1} & \colorbox{green!30}{23.17} &  \colorbox{green!20}{29.6} & \colorbox{red!10}{49.18} \\
    & $dg4$ & 12 & \colorbox{red!30}{628.1} & {112.2} & 129.9 & \colorbox{red!30}{561.9} \\
    & $dg5$ & 14 &  \colorbox{red!30}{to} &  \colorbox{red!30}{to} & \colorbox{green!30}{422.3} &  \colorbox{red!30}{to} \\
    %& $dg10$ & o &  t & m &   t & m &   t & m &   t & m  \\
    %& $dg11$ & o &  t & m &   t & m &   t & m &   t & m  \\
    \toprule
    %---------
    \multirow{3}{*}{Player} & $pl1$ & 2 & 0.069 & 0.06 & 0.065 & 0.63  \\
    & $pl2$ & 9 & \colorbox{red!30}{to} & {215} & \colorbox{red!30}{to} & \colorbox{green!30}{57.22} \\
    & $pl3$ & 12 & \colorbox{red!30}{to} & \colorbox{green!30}{27} & \colorbox{red!30}{to} & {281} \\
    % & $pl4$ & 16 & \colorbox{red!30}{to}  & 1509.6  & \colorbox{red!30}{timeout} & \colorbox{red!30}{timeout} \\
    \toprule
    %---------
    \multirow{5}{*}{PHIM-A} & $pha7$ & 19 & 3.16 & \highlightw{black}{{\textbf{3.37}}} & 3.72 & 3.0\\
    % 14
    & $pha8$ & 23 & 5.0  & 4.4  & 5.3 & 5.4 \\
    & $pha9$ & 26 & 16.5 & 22.2 & 17.6 & 18.1  \\
    %& $pha11$ & 25 & 6.80 & 123 & 7.82 & 126 & 6.63 & 123 & 6.86 & 121 \\
    \bottomrule
    \end{tabular}
    }
    %------------------------ Table 2
    \scalebox{0.75}{
    \begin{tabular}{|c c||c|c|c|c|c|}
    \toprule 
    \multicolumn{2}{|c||}{case studies} & res. & no opt & bcr & %\multicolumn{2}{|c||}{ub} &
    restart & all
    \\ %\toprule 
    \cline{4-5}\cline{6-6}\cline{7-7}
    & & & time & time & time & time \\ \toprule
    %-----------
    
    %-----------
    \multirow{2}{*}{Magic} & 
    %& $m150$ & 4 &  1.83 & 97 & 1.68 & 96 & 1.83 & 98 & 1.82 & 97 & 1.82 & 98 \\ 
    $m300$ & 4 & 1.82 & 1.71 & 1.82 & 1.67 \\ 
    & $m450$ & 4 & 1.83 & 1.72 & 1.82 & 1.68 \\ \toprule
    % ----------
    \multirow{12}{*}{Banking} & 
    %$bd1$ & 5 & 4.79 & 98 & 5.07 & 98 & 5.06 & 102 & 4.78 & 98 & 4.90 & 102 \\
    %& $bd2$ & 7 & 5.51 & 99 & 5.29 & 98 & 7.64 & 111 & 4.76 & 99 & 6.42 & 111 \\
    $bd1$ & \unsat & 1.25 & \colorbox{green!10}{0.84} & 1.85 & \colorbox{red!20}{2.51}  \\
    & $bd2$ &  7 & \colorbox{red!20}{67.55} & \colorbox{red!20}{61.93} & \colorbox{green!30}{8.94} & \colorbox{green!10}{18.36} \\
    & $bd3$ &  12 & \colorbox{red!30}{to} & \colorbox{green!20}{698.2} &  \colorbox{red!30}{to} & \colorbox{green!30}{570.4} \\
    & $bd4$ &  20 & \colorbox{red!30}{to} & \colorbox{green!20}{1544.0} & \colorbox{red!30}{to} &  \colorbox{green!30}{1266} \\
    & $bd5$ & \unsat & \colorbox{red!30}{to} & \colorbox{green!30}{195.3} & \colorbox{red!30}{to} & \colorbox{red!10}{604.55} \\
    % -------------------
    %& $bh1$ &  2 & 0.33 & 83 & 0.33 & 83 &  0.31 & 83 & 0.33 & 83 & 0.32 & 84  \\
    %& $bh2$ &  4 & 1.38 & 92 & 1.33 & 92 & 0.96 & 91 & 1.32 & 92 &  0.92 & 92  \\
    & $bh1$ &  11 &  \colorbox{red!20}{216.99} &  \colorbox{green!23}{55.24} & \colorbox{red!30}{310.26} & \colorbox{green!30}{50.85} \\
    & $bh2$ &  15 & \colorbox{red!10}{128.97} &  \colorbox{green!10}{50.78} & \colorbox{red!20}{161.97} & 76.48 \\
    & $bh3$ &  \unsat & 61.35 & \colorbox{green!30}{3.6} & \colorbox{red!30}{1828} & \colorbox{green!30}{3.7} \\
    & $bh4$ &  17 & \colorbox{red!30}{to}  & 4485 & \colorbox{red!30}{to} & \colorbox{green!30}{3612} \\
    \bottomrule
    \end{tabular}
    }
    \caption{{\footnotesize Effectiveness of \legos{} optimizations on \mfotlplus{} case-studies. Results (res.), running time (time, in seconds) for four settings: only 
    default optimizations (no opt), with 
    bounded case reduction (bcr), with 
    restart (restart), and all optimizations enabled (all). Timeout (to): runtime exceeds 5000 sec. Darker red represents 
    a longer execution time, and darker green---a faster one.}}
    \label{tab:agregation-eval}
    \vspace{-0.25in}
\end{table}
%\end{minipage}







